Evaluating Cosmological Biases using Photometric Redshifts for Type Ia Supernova Cosmology with the Dark Energy Survey Supernova Program

Cosmological analyses with Type Ia Supernovae (SNe Ia) have traditionally been reliant on spectroscopy for both classifying the type of supernova and obtaining reliable redshifts to measure the distance-redshift relation. While obtaining a host-galaxy spectroscopic redshift for most SNe is feasible for small-area transient surveys, it will be too resource intensive for upcoming large-area surveys such as the Vera Rubin Observatory Legacy Survey of Space and Time, which will observe on the order of millions of SNe. Here we use data from the Dark Energy Survey (DES) to address this problem with photometric redshifts (photo-z) inferred directly from the SN light-curve in combination with Gaussian and full p(z) priors from host-galaxy photo-z estimates. Using the DES 5-year photometrically-classified SN sample, we consider several photo-z algorithms as host-galaxy photo-z priors, including the Self-Organizing Map redshifts (SOMPZ), Bayesian Photometric Redshifts (BPZ), and Directional-Neighbourhood Fitting (DNF) redshift estimates employed in the DES 3x2 point analyses. With detailed catalog-level simulations of the DES 5-year sample, we find that the simulated w can be recovered within $\pm$0.02 when using SN+SOMPZ or DNF prior photo-z, smaller than the average statistical uncertainty for these samples of 0.03. With data, we obtain biases in w consistent with simulations within ~1$\sigma$ for three of the five photo-z variants. We further evaluate how photo-z systematics interplay with photometric classification and find classification introduces a subdominant systematic component. This work lays the foundation for next-generation fully photometric SNe Ia cosmological analyses.

==> author_list.tex <==
% Author list file generated with: mkauthlist 1.2.4 
% mkauthlist -f -j mnras --sort-builder --aux order.csv DES-2023-0819_author_list.csv author_list.tex 

\author[DES Collaboration]{
\parbox{\textwidth}{
\Large
R.~Chen,$^{1}$
D.~Scolnic,$^{1}$
M.~Vincenzi,$^{2,3}$
E.~S.~Rykoff,$^{4,5}$
J.~Myles,$^{6}$
R.~Kessler,$^{7,8}$
B.~Popovic,$^{1}$
M.~Sako,$^{9}$
M.~Smith,$^{3}$
P.~Armstrong,$^{10}$
D.~Brout,$^{11,12}$
T.~M.~Davis,$^{13}$
L.~Galbany,$^{14,15}$
J.~Lee,$^{9}$
C.~Lidman,$^{16,10}$
A.~M\"oller,$^{17}$
B.~O.~S\'anchez,$^{1,18}$
M.~Sullivan,$^{3}$
H.~Qu,$^{9}$
P.~Wiseman,$^{3}$
T.~M.~C.~Abbott,$^{19}$
M.~Aguena,$^{20}$
S.~Allam,$^{21}$
O.~Alves,$^{22}$
F.~Andrade-Oliveira,$^{23}$
J.~Annis,$^{21}$
D.~Bacon,$^{2}$
D.~Brooks,$^{24}$
A.~Carnero~Rosell,$^{25,20}$
J.~Carretero,$^{26}$
A.~Choi,$^{27}$
C.~Conselice,$^{28,29}$
L.~N.~da Costa,$^{20}$
M.~E.~S.~Pereira,$^{30}$
H.~T.~Diehl,$^{21}$
P.~Doel,$^{24}$
S.~Everett,$^{31}$
I.~Ferrero,$^{32}$
B.~Flaugher,$^{21}$
J.~Frieman,$^{21,8}$
J.~Garc\'ia-Bellido,$^{33}$
M.~Gatti,$^{9}$
E.~Gaztanaga,$^{14,2,15}$
G.~Giannini,$^{26,8}$
D.~Gruen,$^{34}$
R.~A.~Gruendl,$^{35,36}$
G.~Gutierrez,$^{21}$
K.~Herner,$^{21}$
S.~R.~Hinton,$^{13}$
D.~L.~Hollowood,$^{37}$
K.~Honscheid,$^{38,39}$
D.~Huterer,$^{22}$
D.~J.~James,$^{40}$
K.~Kuehn,$^{41,42}$
M.~Lima,$^{43,20}$
J.~L.~Marshall,$^{44}$
J. Mena-Fern{\'a}ndez,$^{45}$
F.~Menanteau,$^{35,36}$
R.~Miquel,$^{46,26}$
R.~L.~C.~Ogando,$^{47}$
A.~Palmese,$^{48}$
A.~Pieres,$^{20,47}$
A.~A.~Plazas~Malag\'on,$^{4,5}$
A.~Roodman,$^{4,5}$
S.~Samuroff,$^{49}$
E.~Sanchez,$^{50}$
D.~Sanchez Cid,$^{50}$
I.~Sevilla-Noarbe,$^{50}$
E.~Suchyta,$^{51}$
M.~E.~C.~Swanson,$^{35}$
G.~Tarle,$^{22}$
C.~To,$^{38}$
D.~L.~Tucker,$^{21}$
V.~Vikram,$^{9}$
N.~Weaverdyck,$^{52,53}$
and J.~Weller$^{54,55}$
\begin{center} (DES Collaboration) \end{center}
}
\vspace{0.4cm}
\\
\parbox{\textwidth}{
%\scriptsize
$^{1}$ Department of Physics, Duke University Durham, NC 27708, USA\\
$^{2}$ Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK\\
$^{3}$ School of Physics and Astronomy, University of Southampton,  Southampton, SO17 1BJ, UK\\
$^{4}$ Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA\\
$^{5}$ SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA\\
$^{6}$ Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA\\
$^{7}$ Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA\\
$^{8}$ Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{9}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA\\
$^{10}$ The Research School of Astronomy and Astrophysics, Australian National University, ACT 2601, Australia\\
$^{11}$ Department of Astronomy, Boston University, 725 Commonwealth Ave., Boston, MA 02215, USA\\
$^{12}$ Department of Physics, Boston University, 590 Commonwealth Ave., Boston, MA 02215, USA\\
$^{13}$ School of Mathematics and Physics, University of Queensland,  Brisbane, QLD 4072, Australia\\
$^{14}$ Institut d'Estudis Espacials de Catalunya (IEEC), 08034 Barcelona, Spain\\
$^{15}$ Institute of Space Sciences (ICE, CSIC),  Campus UAB, Carrer de Can Magrans, s/n,  08193 Barcelona, Spain\\
$^{16}$ Centre for Gravitational Astrophysics, College of Science, The Australian National University, ACT 2601, Australia\\
$^{17}$ Centre for Astrophysics \& Supercomputing, Swinburne University of Technology, Victoria 3122, Australia\\
$^{18}$ Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France\\
$^{19}$ Cerro Tololo Inter-American Observatory, NSF's National Optical-Infrared Astronomy Research Laboratory, Casilla 603, La Serena, Chile\\
$^{20}$ Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{21}$ Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA\\
$^{22}$ Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA\\
$^{23}$ Physik-Institute, University of Zurich, Winterthurerstrasse 190, 8057 Zurich, Switzerland\\
$^{24}$ Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK\\
$^{25}$ Instituto de Astrofisica de Canarias, E-38205 La Laguna, Tenerife, Spain\\
$^{26}$ Institut de F\'{\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Campus UAB, 08193 Bellaterra (Barcelona) Spain\\
$^{27}$ NASA Goddard Space Flight Center, 8800 Greenbelt Rd, Greenbelt, MD 20771, USA\\
$^{28}$ Jodrell Bank Center for Astrophysics, School of Physics and Astronomy, University of Manchester, Oxford Road, Manchester, M13 9PL, UK\\
$^{29}$ University of Nottingham, School of Physics and Astronomy, Nottingham NG7 2RD, UK\\
$^{30}$ Hamburger Sternwarte, Universit\"{a}t Hamburg, Gojenbergsweg 112, 21029 Hamburg, Germany\\
$^{31}$ Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA\\
$^{32}$ Institute of Theoretical Astrophysics, University of Oslo. P.O. Box 1029 Blindern, NO-0315 Oslo, Norway\\
$^{33}$ Instituto de Fisica Teorica UAM/CSIC, Universidad Autonoma de Madrid, 28049 Madrid, Spain\\
$^{34}$ University Observatory, Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany\\
$^{35}$ Center for Astrophysical Surveys, National Center for Supercomputing Applications, 1205 West Clark St., Urbana, IL 61801, USA\\
$^{36}$ Department of Astronomy, University of Illinois at Urbana-Champaign, 1002 W. Green Street, Urbana, IL 61801, USA\\
$^{37}$ Santa Cruz Institute for Particle Physics, Santa Cruz, CA 95064, USA\\
$^{38}$ Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{39}$ Department of Physics, The Ohio State University, Columbus, OH 43210, USA\\
$^{40}$ Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA\\
$^{41}$ Australian Astronomical Optics, Macquarie University, North Ryde, NSW 2113, Australia\\
$^{42}$ Lowell Observatory, 1400 Mars Hill Rd, Flagstaff, AZ 86001, USA\\
$^{43}$ Departamento de F\'isica Matem\'atica, Instituto de F\'isica, Universidade de S\~ao Paulo, CP 66318, S\~ao Paulo, SP, 05314-970, Brazil\\
$^{44}$ George P. and Cynthia Woods Mitchell Institute for Fundamental Physics and Astronomy, and Department of Physics and Astronomy, Texas A\&M University, College Station, TX 77843,  USA\\
$^{45}$ LPSC Grenoble - 53, Avenue des Martyrs 38026 Grenoble, France\\
$^{46}$ Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, E-08010 Barcelona, Spain\\
$^{47}$ Observat\'orio Nacional, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil\\
$^{48}$ Department of Physics, Carnegie Mellon University, Pittsburgh, Pennsylvania 15312, USA\\
$^{49}$ Department of Physics, Northeastern University, Boston, MA 02115, USA\\
$^{50}$ Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain\\
$^{51}$ Computer Science and Mathematics Division, Oak Ridge National Laboratory, Oak Ridge, TN 37831\\
$^{52}$ Department of Astronomy, University of California, Berkeley,  501 Campbell Hall, Berkeley, CA 94720, USA\\
$^{53}$ Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA 94720, USA\\
$^{54}$ Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany\\
$^{55}$ Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany\\
}
}

